Watch Your Steps: Observable and Modular Chains of Thought

We propose a variant of chain of thought (CoT) prompting called Program Trace Prompting that makes explanations more observable while preserving the power, generality and flexibility of CoT. In our approach, few-shot CoT demonstrations are wrapped in a formal syntax based on Python, and each prompt: identifies and names steps; defines the input/output behavior of steps; and replaces CoT explanations of in-context examples with chains of these formalized steps on the same examples. Program Trace Prompting is applicable to many tasks, achieving strong results on the 23 diverse tasks in the BIG-Bench Hard benchmark. More importantly, by instrumenting explanations in this way, we enable new types of analysis. In particular, we identify "non-local errors" (which correspond to incorrectly learning the reasoning method illustrated in the demonstrations) as an unaddressed issue in CoT learning, and we present methods for verifying the modularity of steps in a CoT explanation.

==> cuts.tex <==
While there is still disagreement over how to define and measure CoT ``faithfulness'', it has been observed that

As we will show below, the prompting scheme of Figure~\ref{fig:fig1} also allows one to generate traces for individual steps, which unlocks new types of analysis.   Here we

\subsubsection{Discussion}

This is another new observation resulting from using \ptp{}, but it is perhaps a little difficult to understand what it implies.   The high performance of step-specific prompts shows that the steps are definitely ``meaningful''---the model ``understands'' then well enough to execute them in a ``step by step'' manner, where each step is performed by an independent LLM call.  However, the improved  performance of steps executed in problem-solving context suggests that LLMs may be using the context, at least in part, to determine what the steps ``mean'' and how to best execute them.  

To summarize, we know that when LLMs perform generation, every token depends in principal on all tokens before it.  However, in \ptp{}, and more generally in CoT reasoning, we hope that generations will not only look like a symbolic explanation, but also behave like it, in that individual reasoning steps are individually justified, and depend on each other in defined ways.  The results of this section suggest that with \ptp{}, LLMs do ``think step by step''---but unlike symbolic explanations, they may be subtly influenced by factors outside a ``step''.  

We explore this question more in the next section.

\newcommand{\fm}{\mathit{ForcedModular}}




As a baseline, we first performed a simpler version of the
measurement method, where we simply truncated the trace $t_i$ after the last line of the $j$-occurrence of step $s$, and then completed that partial trace.  We measured this on all of the dev data, and as expected, there is no significant difference in loss: i.e., completing a trace with the method of Section~\ref{sec:complete-trace} does not significantly change performance.  These results are shown in the first line of Table~\ref{tab:modularity}: breaking a trace after a step and then completing that prefix leads to a different loss 6.4\% of the time, but when the loss changes, it is about as likely to switch from a correct prediction to an error (loss is higher) as to switch from an error to a correct prediction.


\wc{drill down into snarks - overall $p$ = 0.027, judge statement is 0.109, this is not stat significant because of multiple tests, but since only one is sarcastic and judge statement makes that call, seeing the previous judgement would plausibly help.
running snarks on the full test set - another 415 replacements - gives again a small effect. p(change)=10.4\%, p(worse|change) = 58.1\%, p=0.36.}

\begin{table*}
\begin{center}
\begin{small}
   \begin{tabular}{lrcc}
%			& $\Pr(L'_{ij}\not=L_i)$ & $\Pr(L'_{ij} < L_i|L'_{ij}\not=L_i)$ & $p$ value\\
 & $p(\textrm{loss changes})$ & $p(\textrm{loss higher}|\textrm{change})$ & $p$ value \\
   \hline			
   Break and complete (baseline) 	& 6.4\%  & 45.3\% & 0.53 $\gg$ 0.05 \\
   Break, replace and complete
   	  	   	& 10.3\%  & 53.5\% & 0.43 $\gg$ 0.05 \\
   \hline
   \end{tabular}
\end{small}
\end{center}
\caption{Measuring the natural modularity of steps for NLP tasks, by replacing individual steps with versions that are forced to be modular, and testing to see if performance degrades.  Breaking a trace at a step, replacing the step output with a forced-modular version of that step, and then completing the trace after the forced-modular output rarely changes the correctness of the output (10.3\%), and improves results almost as often (46.5\%) as it degrades them (53.5\%).} \label{tab:modularity}
\end{table*}

We thus consider a variant of a  method proposed for studying faithfulness \cite{lanham2023measuring}: the idea is to take a sample of traces and perform an ``intervention'' by changing them in some way, and then measuring the statistical effect of the intervention. For example, one might introduce errors in a CoT explanation and measure the effect on accuracy.  

%, except that they used different sorts of interventions on the trace, and  correctness was used as the only summary statistic $S$.  However, some preliminary experiments we did suggest that the correctness statistic is not ideal.

We thus considered some additional summary statistics $S$ that are designed to detect changed behavior in the trace after step $i$.  In addition to $S_\mathrm{acc}$ (trace correctness), we consider $S_\mathrm{numSteps}$, the number of steps in the trace; and $S_\mathrm{abTrace}$, the abstract trace of Section~\ref{sec:abstract-trace}. %In addition to $S_\mathrm{numSteps}$ we also consider $S_\mathrm{numChars}$, the number of characters in the trace, discretized into the number of length-64 character blocks; we use this as another statistic, like correctness, that could be implemented in a traditional CoT setting.


\subsubsection{Defining modularity} \label{sec:mod-def}

We will model a program trace $t^j$ as a series of steps
$$ f_1^j(x_1^j,y_1^j) \ldots f_n^j(x_n^j, y_n^j) a^j
$$
where each $f_i^j$ is a Python function/step name, $x_i^j$ a tuple of inputs, $y_i^j$ an output (also possibly a tuple), and $a^j$ the final answer produced for the initial CoT input $x^j=x^j_1$.  For brevity we will drop the superscripts when possible.  

Each of the $f_i,x_i,y_i$'s are sequences of tokens generated probabilistically by the LLM in left-to-right order, so we can model the LLM's generations as a joint distribution over variables $F_1,X_1,Y_1,\ldots,F_n,X_n,Y_n,A$. Then each $y_i$ depends on the preceding sequence, which we write:
\begin{equation} \label{eq:l2r}
    y_i \sim P(Y_i|
% F_{\leq{}i}=f_{\leq{}i},X_{\leq{}i}=x_{\leq{}i},Y_{<i}=y_{<i})
 F_{\leq{}i},X_{\leq{}i},Y_{<i})
\end{equation}
where $X_{\leq{}i}$ is shorthand for $X_1,\ldots,X_{i}$, and so on.

Equation~\ref{eq:l2r} holds for any LLM, but the trace syntax we used additionally suggests that the $f_i$'s act like actual Python functions, where $y_i$ depends only on $f_i$ and $x_i$:
$$
y_i \sim P(Y_i | F_{i}=f_i,X_{i}=x_i)
$$
In other words, %the step-by-step nature of the traces suggest that 
each $Y_i$ is conditionally independent of everything else given $X_i$ and $F_i$, i.e.
\begin{equation} \label{eq:indep}
    P(Y_i | F_{i},X_{i}) = P(Y_i | F_{\leq{}i},X_{\leq{}i},Y_{<i})
\end{equation}
The experiments of Section~\ref{sec:oracle} also make this assumption (since the oracle's result depends only on its inputs).

We define step $i$ to be \emph{modular} if and only iff Equation~\ref{eq:indep} holds.  For example, in the trace of Figure~\ref{fig:fig1}, the step \wctt{sport\_for} is modular if the output of calling this step with the input string \wctt{'scored a touchdown'} depends only on that input, and is not influenced by anything else in the trace.

We use the formal notion of step modularity to approximate the informal notions of a step being ``meaningful'', and an model ``thinking step by step''.   To justify this, notice that
when Equation~\ref{eq:indep} holds, $f_i$ is interpretable, in that it always generates a $y_i$ according to a the input $x_i$.  Conversely when Equation~\ref{eq:indep} does \emph{not} hold, then $f_i$ is difficult to interpret, since it might do something different in different contexts.
If all steps are modular, then generation is arguably a ``step by step'' process, in the precise sense that the $i$-th output $y_i$ depends only on (1) the choice of what step $f_i$ to use and (2) the selection of the inputs $x_i$ for that step.\footnote{Of course, if a non-local error occurs, the choice of step $f_i$ or input $x_i$ might be wrong.}

\subsubsection{Measuring modularity by forcing modular behavior} \label{sec:mod-measure}

To measure modularity, we adapt an approach proposed by \cite{lanham2023measuring} to measure faithfulness, in which one measures the impact on reasoning of \emph{interventions} that modify a CoT explanation.  Our intervention is to \emph{force a particular step to be modular}, by replacing its output with the result of a single-step prompt of the same function $f_i$ on the same input $x_i$.  After making this change, we then extend the resulting trace prefix using the method of Section~\ref{sec:complete-trace}.  Precisely, if $i$ is the position of the designated step in the trace $t$
$$ t = f_1(x_1,y_1) \ldots f_i(x_i, y_i) \ldots f_n(x_n,y_n) a
$$
then we replace $y_i$ with a new value $\tilde{y}_i$ produced with a single step prompt
$$ \tilde{y_i} \sim P(Y_i | F_i=f_i, X_i=x_i)
$$
We then ask the LLM to predict the rest of the trace, which will potentially change every subsequent $x$, $f$, and $y$, yielding the new trace
$$
\tilde{t} = f_1(x_1,y_1) \ldots f_i(x_i, 
            \tilde{y}_i) \ldots \tilde{f}_n(\tilde{x}_n,\tilde{y}_n) \tilde{a}
$$

Let $P({T}|X_1=x_1)$ be the distribution of traces produced from input $x_1$, and let $P(\tilde{T}|X_1=x_1)$ be the distribution of  traces after this intervention. Assume that the step of completing a a trace prefix does not change the distribution: i.e., that 
\begin{eqnarray}
 \lefteqn{P(T|X_1=x_1) = } \nonumber \\
 && P(T|F_1,Y_1,\ldots,F_i,X_i,Y_i) \cdot \label{eq:pref} \\
 &&                 P(F_1,Y_1,\ldots,F_i,X_i,Y_i|X_1=x_1) \label{eq:cont}
\end{eqnarray}
where line~\ref{eq:pref} is sampled by producing an entire trace and picking the first $i$ steps, and line~\ref{eq:cont} is sampled by
completing the trace.  Below we call this assumption the \emph{stable incremental generation assumption:} it holds for a traditional left-to-right LM, but may not for the prompted trace-completion strategy we use. If incremental generation holds, and step $i$ is modular, then $P(\tilde{T}|X_1) = P(T|X_1)$.  

Similarly, suppose $S$ is any summary statistic derived from a trace, i.e.
$s \sim{} P(S|T)$.
For example, $S$ could be the length of the trace or the correctness of the trace. (When $S$ is just a deterministic function of $T$ we also write this as $s=g_s(T)$.) If we assume stable incremental generation, then if step $i$ is modular this also implies 
$$P(\tilde{S}|X_1) = P(S|X_1)$$
This means \emph{we can detect failures in modularity if we can detect changes in the distribution of the distributions of the statistics $S$ and $\tilde{S}$}, using the forced-modularity intervention described above.

Specifically, in the experiments below, we take a sample of $m$ inputs $\mathcal{X}_1=\{x_1^1,\ldots,x_1^m\}$ and compute corresponding samples of the summary statistics 
$\mathcal{S}=\{g_s(t^1, \ldots, g_s(t^m)\}$ and 
$\tilde{\mathcal{S}}=\{g_s(\tilde{t}^1, \ldots, g_s(\tilde{t}^m)\}$.  We test if the Jensen-Shannon divergence between $S$ and $\tilde{S}$ is higher than expected using a permutation test (see Section~\ref{app:stats}).  


\iffalse
Intervention			& $P(\tilde{C}\not=C)$	& $P(\tilde{C}=0 | \tilde{C}\not=C)$ \\
Split at $i$ and continue trace	  		& 7.1\% & 47.2\% $(n=72, k=34)$ \\
Split at $i$, force modularity, continue	& 10.5\% & 49.5\% $(n=105, k=52)$ \\

$p$-values < 0.1:
 snarks, summarize\_statement, $p=0.03$
\fi





